Astrometric and photometric standard candidates for the upcoming 4-m ILMT survey

The International Liquid Mirror Telescope (ILMT) is a 4-meter class survey telescope that has recently achieved first light and is expected to swing into full operations by 1st January 2023. It scans the sky in a fixed 22' wide strip centered at the declination of $+29^o21'41''$ and works in Time Delay Integration (TDI) mode. We present a full catalog of sources in the ILMT strip that can serve as astrometric calibrators. The characteristics of the sources for astrometric calibration are extracted from Gaia EDR3 as it provides a very precise measurement of astrometric properties such as RA ($\alpha$), Dec ($\delta$), parallax ($\pi$), and proper motions ($\mu_{\alpha^{*}}$ & $\mu_{\delta}$). We have crossmatched the Gaia EDR3 with SDSS DR17 and PanSTARRS-1 (PS1) and supplemented the catalog with apparent magnitudes of these sources in g, r, and i filters. We also present a catalog of spectroscopically confirmed white dwarfs with SDSS magnitudes that may serve as photometric calibrators. The catalogs generated are stored in a SQLite database for query-based access. We also report the offsets in equatorial positions compared to Gaia for an astrometrically calibrated TDI frame observed with the ILMT.

==> tables/gaia_filter.tex <==
\begin{table}
\centering
\caption{Summary of \textit{Gaia} objects at different part of the filtering.}
\begin{tabular}{cc} 
\hline
No of \textit{Gaia} sources in the initial sample & 7,621,343 \\
sources left after $parallax < 10\, mas$ filter & 6,610,739 \\
sources left after $pm < 20\, mas/yr$ filter & 6,438,173 \\
sources left after $D < 2$ filter & 5,462,888 \\ \hline
\end{tabular}
\label{tab:gaia_filter}
\end{table}

